Superconductivity of alpha-gallium probed on the atomic scale by normal and Josephson tunneling

We investigate superconducting gallium in its $\alpha$ phase using scanning tunneling microscopy and spectroscopy at temperatures down to about 100 mK. High-resolution tunneling spectroscopies using both superconducting and normal tips show that superconducting $\alpha$-Ga is accurately described by Bardeen-Cooper-Schrieffer theory, with a gap $\Delta_{\rm Ga}$ = 163 $\mu$eV on the $\alpha-$Ga(112) facet, with highly homogeneous spectra over the surface, including atomic defects and step edges. Using a superconducting Pb tip, we furthermore study the low-bias conductance features of the Josephson junction formed between tip and sample. The features are accurately described by dynamical Coulomb blockade theory, highlighting $\alpha-$Ga as a possible platform for surface science studies of mesoscopic superconductivity.

==> random_Corinna.tex <==
%previous studies of the alpha-Ga surface
[33] M. Bernasconi, G. L. Chiarotti, and E. Tosatti, “Theory of the structural and electronic
properties of α-Ga (001) and (010) surfaces,” Physical Review B, vol. 52, no. 14,
p. 9999, 1995.
[34] O. Züger and U. Dürig, “STM investigation of gallium single-crystal surfaces close
to bulk melting,” Ultramicroscopy, vol. 42, pp. 520–527, 1992.
